Multi-Head Adapter Routing for Cross-Task Generalization

Parameter-efficient fine-tuning (PEFT) for cross-task generalization consists in pre-training adapters on a multi-task training set before few-shot adaptation to test tasks. Polytropon [Ponti et al., 2023] ($\texttt{Poly}$) jointly learns an inventory of adapters and a routing function that selects a (variable-size) subset of adapters for each task during both pre-training and few-shot adaptation. In this paper, we investigate the role that adapter routing plays in its success and design new variants based on our findings. First, we build on the intuition that finer-grained routing provides more expressivity. Hence, we propose $\texttt{MHR}$ (Multi-Head Routing) which combines subsets of adapter parameters and outperforms $\texttt{Poly}$ under a comparable parameter budget; by only fine-tuning the routing function and not the adapters ($\texttt{MHR}$-$z$) we achieve competitive performance with extreme parameter efficiency. Second, we find that $\texttt{Poly}$/$\texttt{MHR}$ performance is a result of better multi-task optimization, rather than modular inductive biases that facilitate adapter recombination and local adaptation, as previously hypothesized. In fact, we find that $\texttt{MHR}$ exhibits high gradient alignment between training tasks. We find that routing is most beneficial during multi-task pre-training rather than during few-shot adaptation and propose $\texttt{MHR}$-$\mu$, which discards routing and fine-tunes the average of the pre-trained adapters on each downstream tasks. This establishes $\texttt{MHR}$-$\mu$ as an effective method for single-adapter fine-tuning. We also show that $\texttt{MHR}$-$\mu$ can be used as an effective zero-shot transfer method by training the average of the pre-trained adapters for a few additional steps on the multi-task training set: this yields gains up to 3% on absolute accuracy w.r.t. the baselines.

==> notes.tex <==

  Lucas Caccia\footnote{correspoonding author \texttt{lucas.page-caccia@mail.mcgill.ca}} \\
  Microsoft Research\\
  McGill University, Mila\\
  \And
  Edoardo Ponti\\
  University of Edinburgh\\
  University of Cambridge \\
  % examples of more authors
  \AND
  \hspace{-5pt} Lucas Liu \\
  \hspace{-5pt} Microsoft Research\\
  \And
  \hspace{8pt} Matheus Pereira\\
  \hspace{8pt} Microsoft Research\\
  \AND
  \hspace{6pt} Nicolas Le Roux\\
  \hspace{6pt}  Microsoft Research\\
  \hspace{6pt}  McGill University, Mila\\
  \And
  Alessandro Sordoni\\
  Microsoft Research\\
  Universit\'e de Montr\'eal, Mila\\
  \AND
}

==> old_tables/mix_table.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lc|cc|l}
\toprule
Dataset & \texttt{Shared} & \texttt{Poly}-$\mu$ & \texttt{Poly} & \texttt{Poly}-$S$ \\
\midrule
Natural Instructions Avg. & 64.9$_{0.5}$ & 65.9$_{0.7}$ & 67.2$_{0.7}$ & \underline{70.2}$_{0.4}$ (+5.3) \\
\midrule
T0 tasks Avg.$^*$ &  66.9$_{0.7}$  & 67.2$_{1.1}$  & 67.1$_{1.4}$ & \underline{67.5}$_{0.5}$ (+0.6)
\\
\bottomrule
\end{tabular}
\caption{Few-shot results on Natural Instructions (NI) and the T0 dataset. For T0, \shared{} corresponds to \texttt{T-Few}~\cite{tfew}. \texttt{Poly}-$\mu$ is more performant than \texttt{Shared}, showing that average initialization is useful. In Natural Instructions, \texttt{Poly} outperforms both approaches, suggesting that the skills specialize and exploit NI task diversity. In both datasets,~\polys{} substantially improve over all baselines.} 
\label{tab:mix}
\end{table*}


==> old_tables/new_ni_table.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lcc|ccc}
\toprule
& \texttt{Shared-ia3} & \texttt{Shared} & \texttt{Poly}-$\mu$ & \texttt{Poly} & \texttt{Poly}-$S$ \\
\midrule
\textsc{wino. question modification person} & 90.8$_{0.0}$ & 90.9$_{0.1}$ & 90.8$_{0.1}$ & 90.9$_{0.2}$ & 90.9$_{0.0}$ \\
\textsc{bard anal. reasoning causation} &  2.0$_{0.0}$ &  99.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$  \\
\textsc{bard anal. reasoning travel}  &  39.0$_{1.0}$ &  93.7$_{0.6}$ & 93.7$_{3.5}$ & 96.0$_{0.0}$ & 98.3$_{0.6}$ \\
\textsc{bard anal. reasoning rooms cont.}  &  80.0$_{0.0}$ &  94.0$_{1.0}$ & 93.7$_{1.2}$ & 94.0$_{1.0}$ & 94.0$_{1.0}$ \\
\textsc{xlsum title generation} &  29.2$_{0.1}$ &  33.8$_{0.1}$ & 34.2$_{0.7}$ & 33.0$_{0.5}$ & 
34.4$_{0.1}$
\\
\textsc{anli r1 entailment} &  37.0$_{1.7}$ &  31.0$_{2.6}$ & 33.3$_{1.5}$ & 31.7$_{1.2}$ &
31.7$_{1.5}$ \\
\textsc{superglue copa text completion} &  57.3$_{0.6}$ &  51.0$_{6.0}$ & 62.3$_{1.5}$ & 68.7$_{1.2}$ &
74.0$_{1.0}$ \\
\textsc{daily dialog type classification} &  40.0$_{0.9}$ &  66.0$_{1.0}$ & 63.3$_{2.9}$ & 66.3$_{0.6}$ &
64.3$_{3.2}$\\
\textsc{nyc long text generation} &  41.0$_{0.1}$ &  47.9$_{1.1}$ & 46.4$_{1.0}$ & 46.2$_{1.4}$ &
46.4$_{0.6}$ \\
\textsc{disfl qa text modication}  &  81.2$_{0.2}$ &  90.9$_{0.4}$ & 90.5$_{0.4}$ & 92.2$_{0.1}$ &
91.9$_{0.6}$  \\
\textsc{disfl qa quest. yesno class.} &  50.0$_{2.6}$ &  68.0$_{2.6}$ & 67.0$_{11.3}$ & 66.3$_{10.7}$ &
 78.3$_{3.1}$ \\
\textsc{mnli neutral class.} &  24.7$_{0.6}$ &  37.0$_{1.7}$ & 45.3$_{3.5}$ & 51.0$_{2.6}$ &
79.0$_{4.0}$ \\
\textsc{ambigqa text generation} &  67.2$_{0.0}$ &  67.0$_{0.0}$ & 67.4$_{0.3}$ & 68.1$_{0.0}$ &
68.2$_{0.0}$  \\
\textsc{ollie sentence answer generation}  &  19.9$_{0.1}$ &  30.0$_{0.1}$ & 29.5$_{0.2}$ & 30.1$_{0.8}$ &
29.4$_{0.7}$ \\
\textsc{schema guided dstc8 class.}  &  46.0$_{2.1}$ &  88.1$_{0.8}$ & 85.8$_{1.8}$ & 89.4$_{0.7}$ &
92.0$_{0.9}$ \\
\textsc{e2e nlg text generation generate} &  47.7$_{0.3}$ &  50.1$_{0.3}$ & 50.4$_{0.3}$ & 50.7$_{0.6}$ &
50.7$_{0.8}$ \\
\midrule
Avg & 47.1$_{0.1}$ & 64.9$_{0.5}$ & 65.9$_{0.7}$ & 67.2$_{0.7}$ & \textbf{70.2}$_{0.4}$ \\
\bottomrule
\end{tabular}
\caption{Few-shot results on Natural Instructions (NI). \texttt{Poly}-$\mu$ is more performant than \texttt{Shared}, confirming that average initialization is useful. \texttt{Poly} outperforms both approaches, illustrating that the learnt skills specialize and exploit task diversity during pre-training. \polys{} substantially improve over all baselines. We also try to parametrize skills with \texttt{ia3}: in this case, we obtain a significant lower performance than by using LoRA.}
\label{tab:ni_old}
\end{table*}


==> old_tables/ni_table.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lcc|c|cl}
\toprule
& \texttt{Shared[ia3]} & \texttt{Shared} & \texttt{Poly}-$\mu$ & \texttt{Poly} & \texttt{Poly}-$S$ \\
\midrule
Avg. & 47.1$_{0.1}$ & 64.9$_{0.5}$ & 65.9$_{0.7}$ & 67.2$_{0.7}$ & \textbf{70.2}$_{0.4}$ (+5.3) \\
\bottomrule
\end{tabular}
\caption{Few-shot results on Natural Instructions (NI). \texttt{Poly}-$\mu$ is more performant than \texttt{Shared}, showing that average initialization is useful. \texttt{Poly} outperforms both approaches, illustrating that the modules specialize and exploit task diversity during pre-training. \polys{} substantially improve over all baselines. Using IA3 seems to lead to significant lower performance than by using LoRA.}
\label{tab:ni}
\end{table*}


==> old_tables/noia3_ni_table.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lc|r|rrr}
\toprule
NI Task & \texttt{Shared} & \fullft{} & \texttt{Poly}-$\mu$ & \texttt{Poly} & \texttt{Poly}-$S$ \\
\midrule
\textsc{wino. question modification person} & 90.9$_{0.1}$ & 91.1$_{0.1}$ & 90.8$_{0.1}$ & 90.9$_{0.2}$ & 90.9$_{0.0}$ \\
\textsc{bard anal. reasoning causation} & 99.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$  \\
\textsc{bard anal. reasoning travel}  &   93.7$_{0.6}$ & 100.0$_{0.0}$ & 93.7$_{3.5}$ & 96.0$_{0.0}$ & 98.3$_{0.6}$ \\
\textsc{bard anal. reasoning rooms cont.}  &   94.0$_{1.0}$ & 99.0$_{0.0}$ & 93.7$_{1.2}$ & 94.0$_{1.0}$ & 94.0$_{1.0}$ \\
\textsc{xlsum title generation} &  33.8$_{0.1}$ &31.8$_{1.2}$  & 34.2$_{0.7}$ & 33.0$_{0.5}$ & 
34.4$_{0.1}$
\\
\textsc{anli r1 entailment} &    31.0$_{2.6}$ & 40.0$_{6.1}$ & 33.3$_{1.5}$ & 31.7$_{1.2}$ &
31.7$_{1.5}$ \\
\textsc{superglue copa text completion} &   51.0$_{6.0}$ &51.7$_{2.5}$ & 62.3$_{1.5}$ & 68.7$_{1.2}$ &
74.0$_{1.0}$ \\
\textsc{daily dialog type classification} &   66.0$_{1.0}$ &61.7$_{2.5}$ & 63.3$_{2.9}$ & 66.3$_{0.6}$ &
64.3$_{3.2}$\\
\textsc{nyc long text generation} &    47.9$_{1.1}$ &49.6$_{0.1}$ & 46.4$_{1.0}$ & 46.2$_{1.4}$ &
46.4$_{0.6}$ \\
\textsc{disfl qa text modication}  &  90.9$_{0.4}$ & 89.2$_{0.6}$& 90.5$_{0.4}$ & 92.2$_{0.1}$ &
91.9$_{0.6}$  \\
\textsc{disfl qa quest. yesno classification} & 68.0$_{2.6}$ & 63.0$_{11.3}$& 67.0$_{11.3}$ & 66.3$_{10.7}$ &
 78.3$_{3.1}$ \\
\textsc{mnli neutral classification} &  37.0$_{1.7}$ & 51.7$_{5.0}$ & 45.3$_{3.5}$ & 51.0$_{2.6}$ &
79.0$_{4.0}$ \\
\textsc{ambigqa text generation} &   67.0$_{0.0}$ &59.6$_{0.3}$ & 67.4$_{0.3}$ & 68.1$_{0.0}$ &
68.2$_{0.0}$  \\
\textsc{ollie sentence answer generation}  &    30.0$_{0.1}$ & 27.0$_{0.2}$& 29.5$_{0.2}$ & 30.1$_{0.8}$ &
29.4$_{0.7}$ \\
\textsc{schema guided dstc8 classification}  &    88.1$_{0.8}$ & 92.8$_{3.9}$ & 85.8$_{1.8}$ & 89.4$_{0.7}$ &
92.0$_{0.9}$ \\
\textsc{e2e nlg text generation generate} &    50.1$_{0.3}$ & 49.2$_{1.2}$ & 50.4$_{0.3}$ & 50.7$_{0.6}$ &
50.7$_{0.8}$ \\
\midrule
Avg & 64.9$_{0.5}$ & 66.1$_{0.4}$ & 65.9$_{0.7}$ & 67.2$_{0.7}$ & \underline{70.2}$^{\uparrow5.3}_{0.4}$ \\
\bottomrule
\end{tabular}
\caption{Few-shot results on a subset of 16 tasks from Natural Instructions (NI) test set. \texttt{Shared} corresponds to multi-task pre-training one adapter on $\mathcal{T}_{train}$ and fine-tuning its parameters for each task in $\mathcal{T}_{eval}$. \fullft{} is similar but we multi-task train and fine-tune all parameters of the pre-trained T5-Large. \texttt{Poly}-$\mu$ is more performant than \texttt{LoRA}, confirming that averaging Polytropon's skills is a better initialization. \texttt{Poly} outperforms both approaches, illustrating that the learnt skills specialize and exploit task diversity during pre-training. \polys{} substantially improve over all baselines.}
\label{tab:ni}
\end{table*}


==> old_tables/old_ni_table.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lcc|ccc}
\toprule
& \texttt{Shared-ia3} & \texttt{Shared} & \texttt{Poly}-$\mu$ & \texttt{Poly} & \texttt{Poly}-$S$ \\
\midrule
\textsc{wino. question modification person} & 90.8$_{0.0}$ & 90.9$_{0.1}$ & 90.8$_{0.1}$ & 90.9$_{0.2}$ & 90.9$_{0.0}$ \\
\textsc{bard anal. reasoning causation} &  2.0$_{0.0}$ &  99.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$ & 100.0$_{0.0}$  \\
\textsc{bard anal. reasoning travel}  &  39.0$_{1.0}$ &  93.7$_{0.6}$ & 93.7$_{3.5}$ & 96.0$_{0.0}$ & 98.3$_{0.6}$ \\
\textsc{bard anal. reasoning rooms cont.}  &  80.0$_{0.0}$ &  94.0$_{1.0}$ & 93.7$_{1.2}$ & 94.0$_{1.0}$ & 94.0$_{1.0}$ \\
\textsc{xlsum title generation} &  29.2$_{0.1}$ &  33.8$_{0.1}$ & 34.2$_{0.7}$ & 33.0$_{0.5}$ & 
34.4$_{0.1}$
\\
\textsc{anli r1 entailment} &  37.0$_{1.7}$ &  31.0$_{2.6}$ & 33.3$_{1.5}$ & 31.7$_{1.2}$ &
31.7$_{1.5}$ \\
\textsc{superglue copa text completion} &  57.3$_{0.6}$ &  51.0$_{6.0}$ & 62.3$_{1.5}$ & 68.7$_{1.2}$ &
74.0$_{1.0}$ \\
\textsc{daily dialog type classification} &  40.0$_{0.9}$ &  66.0$_{1.0}$ & 63.3$_{2.9}$ & 66.3$_{0.6}$ &
64.3$_{3.2}$\\
\textsc{nyc long text generation} &  41.0$_{0.1}$ &  47.9$_{1.1}$ & 46.4$_{1.0}$ & 46.2$_{1.4}$ &
46.4$_{0.6}$ \\
\textsc{disfl qa text modication}  &  81.2$_{0.2}$ &  90.9$_{0.4}$ & 90.5$_{0.4}$ & 92.2$_{0.1}$ &
91.9$_{0.6}$  \\
\textsc{disfl qa quest. yesno class.} &  50.0$_{2.6}$ &  68.0$_{2.6}$ & 67.0$_{11.3}$ & 66.3$_{10.7}$ &
 78.3$_{3.1}$ \\
\textsc{mnli neutral class.} &  24.7$_{0.6}$ &  37.0$_{1.7}$ & 45.3$_{3.5}$ & 51.0$_{2.6}$ &
79.0$_{4.0}$ \\
\textsc{ambigqa text generation} &  67.2$_{0.0}$ &  67.0$_{0.0}$ & 67.4$_{0.3}$ & 68.1$_{0.0}$ &
68.2$_{0.0}$  \\
\textsc{ollie sentence answer generation}  &  19.9$_{0.1}$ &  30.0$_{0.1}$ & 29.5$_{0.2}$ & 30.1$_{0.8}$ &
29.4$_{0.7}$ \\
\textsc{schema guided dstc8 class.}  &  46.0$_{2.1}$ &  88.1$_{0.8}$ & 85.8$_{1.8}$ & 89.4$_{0.7}$ &
92.0$_{0.9}$ \\
\textsc{e2e nlg text generation generate} &  47.7$_{0.3}$ &  50.1$_{0.3}$ & 50.4$_{0.3}$ & 50.7$_{0.6}$ &
50.7$_{0.8}$ \\
\midrule
Avg & 47.1$_{0.1}$ & 64.9$_{0.5}$ & 65.9$_{0.7}$ & 67.2$_{0.7}$ & \textbf{70.2}$_{0.4}$ \\
\bottomrule
\end{tabular}
\caption{Few-shot results on the test set of 16 test tasks of the Natural Instructions (NI) dataset. The base model is T5-Large. \texttt{Poly}-$\mu$ is more performant than \texttt{Shared}, showing that average initialization is useful. In this case, \texttt{Poly} outperforms both approaches, illustrating that the modules might be specializing and exploiting task diversity during pre-training. We also try to parametrize skills with \texttt{ia3}: in this case, we obtain a significant lower performance than by using LoRA.}
\label{tab:ni_old}
\end{table*}


==> old_tables/old_t0_table.tex <==
\begin{table*}
\centering
\begin{tabular}{lccccccccc}
\toprule
&&\texttt{0-shot} & &&& &\texttt{few-shot}$^*$ & \vspace{1mm} \\
\midrule
Dataset & \texttt{Poly} & \texttt{Poly}-$\mu$ & \shared{}  &&& \texttt{Poly} & \texttt{Poly}-$\mu$ & \shared{} \\
\midrule
\textsc{anli-r1} & $37.2_{0.7}$&$36.9_{0.8}$&$37.9_{0.8}$ &&& $46.5_{2.1}$&$45.9_{4.9}$&$47.2_{4.1}$\\
\textsc{anli-r2} & $36.8_{0.3}$&$37.2_{0.3}$&$36.9_{0.8}$ &&& $40.9_{1.3}$&$40.7_{1.5}$&$42.0_{1.6}$\\
\textsc{anli-r3} & $36.0_{0.4}$&$35.8_{0.4}$&$36.0_{0.4}$ &&& $38.9_{3.7}$&$41.2_{3.2}$&$40.9_{3.6}$\\
\textsc{cb} & $53.6_{8.9}$&$53.6_{5.4}$&$46.4_{5.4}$ &&& $87.5_{3.6}$&$85.7_{3.6}$&$87.5_{1.8}$\\
\textsc{copa} & $84.0_{5.0}$&$83.0_{5.0}$&$82.0_{1.0}$ &&& $83.0_{7.0}$&$87.0_{6.0}$&$88.0_{6.0}$\\
\textsc{h-swag} & $27.6_{0.0}$&$27.6_{0.2}$&$27.0_{0.5}$ &&& $52.2_{1.0}$&$51.8_{0.3}$&$51.6_{3.9}$\\
\textsc{rte} & $76.9_{0.7}$&$76.9_{1.1}$&$74.4_{1.8}$ &&& $80.1_{1.4}$&$83.8_{2.9}$&$78.7_{3.2}$\\
\textsc{storycloze} & $90.2_{0.1}$&$90.1_{0.1}$&$89.8_{0.1}$ &&& $93.5_{2.5}$&$93.9_{2.2}$&$95.0_{1.8}$\\
\textsc{wic} & $51.9_{0.8}$&$51.4_{0.8}$&$51.7_{0.9}$ &&& $55.6_{3.0}$&$57.2_{1.4}$&$56.4_{3.1}$\\
\textsc{winogrande} & $51.9_{0.6}$&$51.9_{0.7}$&$51.1_{1.0}$ &&& $62.9_{1.2}$&$62.7_{0.6}$&$62.3_{1.2}$\\
\textsc{wsc} & $63.5_{4.8}$&$63.5_{3.8}$&$64.4_{6.7}$ &&& $68.3_{3.8}$&$67.3_{1.9}$&$67.3_{4.8}$\\
\midrule
Avg & \textbf{55.4} & 55.3 &54.3  &&& 64.5 & \textbf{65.2} & 65.2 &\\
\bottomrule
\end{tabular}
\caption{Results in the $\texttt{zero-shot}$ and $\texttt{few-shot}$ setting for the T0 dataset. The asterisk is meant to denote that we fine-tune all models for 1000 steps on the training set of the test tasks, given the lack of a validation set. This setting is the default in the \texttt{T-Few} paper and thus we suspect it benefits \texttt{T-Few}.}
% \end{tabular}
\end{table*}

==> old_tables/old_xfit_bigtable.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{ll|r|rrrrrr}


\toprule
Task & Metric & \texttt{Poly} & \texttt{Poly}-$\mu$ & \texttt{Shared} & \texttt{Random}-$\mu$ & \texttt{Private}-$\mu$ \\
\midrule
\textsc{ag-news} & \textsc{C--F1} & 85.0$_{2.1}$ &85.1$_{1.3}$ &81.5$_{1.3}$ &83.3$_{2.3}$ &71.3$_{7.1}$ \\
\textsc{ai2-arc} & \textsc{Acc} & 24.0$_{2.2}$ &24.2$_{3.3}$ &27.2$_{2.1}$ &24.7$_{1.3}$ &22.9$_{2.4}$ \\
\textsc{amazon-polarity} & \textsc{C--F1} & 92.7$_{1.9}$ &92.4$_{2.0}$ &87.6$_{14.4}$ &93.0$_{0.8}$ &78.5$_{22.5}$ \\
\textsc{bsn-npi-present} & \textsc{Acc} & 99.1$_{0.5}$ &99.6$_{0.2}$ &99.2$_{0.4}$ &99.2$_{0.4}$ &100.0$_{0.0}$ \\
\textsc{bsn-npi-scope} & \textsc{Acc} & 99.6$_{0.7}$ &99.4$_{0.9}$ &99.9$_{0.2}$ &100.0$_{0.0}$ &99.6$_{0.9}$ \\
\textsc{break-QDMR} & \textsc{EM} & 4.1$_{0.5}$ &3.5$_{1.0}$ &3.9$_{0.8}$ &2.6$_{1.5}$ &3.0$_{1.5}$ \\
\textsc{circa} & \textsc{C--F1} & 43.5$_{6.4}$ &45.4$_{4.7}$ &46.4$_{4.7}$ &47.3$_{5.2}$ &31.2$_{7.9}$ \\
\textsc{crawl-domain} & \textsc{EM} & 45.0$_{4.2}$ &47.3$_{1.3}$ &40.0$_{3.0}$ &43.9$_{2.0}$ &42.9$_{3.7}$ \\
\textsc{ethos-disability} & \textsc{C--F1} & 74.0$_{10.3}$ &73.4$_{9.8}$ &69.9$_{9.9}$ &60.6$_{8.6}$ &54.0$_{6.5}$ \\
\textsc{ethos-sexual} & \textsc{C--F1} & 78.9$_{4.5}$ &81.4$_{9.6}$ &65.0$_{9.7}$ &58.9$_{16.1}$ &52.3$_{15.5}$ \\
\textsc{freebase-qa} & \textsc{EM} & 3.8$_{1.5}$ &3.9$_{1.7}$ &2.7$_{1.0}$ &5.4$_{0.6}$ &0.1$_{0.2}$ \\
\textsc{glue-cola} & \textsc{M-Corr} & 7.5$_{11.6}$ &8.2$_{5.6}$ &6.8$_{4.4}$ &7.9$_{6.8}$ &9.5$_{5.7}$ \\
\textsc{glue-qnli} & \textsc{Acc} & 73.1$_{4.4}$ &72.3$_{5.0}$ &74.0$_{2.4}$ &75.2$_{3.4}$ &55.3$_{2.8}$ \\
\textsc{hatexplain} & \textsc{C--F1} & 44.3$_{2.5}$ &42.2$_{4.1}$ &43.6$_{3.3}$ &43.8$_{2.4}$ &33.3$_{3.9}$ \\
\textsc{quoref} & \textsc{QA--F1} & 45.0$_{3.9}$ &46.3$_{2.2}$ &43.8$_{2.8}$ &44.6$_{4.3}$ &33.5$_{3.1}$ \\
\textsc{race-high} & \textsc{Acc} & 32.4$_{1.5}$ &33.0$_{0.7}$ &34.9$_{1.0}$ &34.0$_{2.9}$ &26.0$_{1.7}$ \\
\textsc{superglue-rte} & \textsc{Acc} & 52.3$_{3.8}$ &52.0$_{3.3}$ &60.1$_{3.2}$ &57.7$_{3.7}$ &47.8$_{2.2}$ \\
\textsc{tweet-eval-irony} & \textsc{C--F1} & 54.8$_{1.7}$ &55.6$_{1.4}$ &56.7$_{3.0}$ &57.2$_{2.2}$ &46.0$_{7.5}$ \\
\textsc{wiki-split} & \textsc{Rouge-L} & 80.2$_{0.3}$ &79.8$_{1.0}$ &80.3$_{0.5}$ &80.3$_{0.5}$ &80.7$_{0.3}$ \\
\textsc{yelp-polarity} & \textsc{C--F1} & 94.9$_{0.4}$ &95.1$_{0.5}$ &94.8$_{0.8}$ &94.4$_{0.4}$ &55.2$_{11.9}$ \\
\midrule
All & Avg & 56.7$_{1.0}$ & \textbf{57.0}$_{0.6}$ &55.9$_{0.8}$ &55.7$_{0.6}$ &47.2$_{1.4}$ \\
\bottomrule

\end{tabular}
\caption{\small Few-shot results on the 20 \texttt{CrossFit} test tasks obtained by fine-tuning Polytropon (\texttt{Poly}, learns both weights $\hat z$ and skills $\Phi$), \polym{} (fine-tunes the average of skills learnt during Polytropon pre-training), \texttt{Shared} (fine-tunes one shared skill learnt during pre-training), \texttt{Random}-$\mu$ (fine-tunes the average of skills learnt during training with a random fixed $Z$) and \texttt{Private}-$\mu$ (fine-tunes the average of private skills, one per training task). In \texttt{CrossFit}, most of the \texttt{Poly} gain comes from the effective initialization while the tuning of the skill-allocation vector $\hat z$ for the downstream tasks seems unnecessary.}

\label{tab:ft}
\vspace{-2mm}
\end{table*}

==> old_tables/oldish_t0_table.tex <==
\begin{table*}
\centering
\begin{tabular}{lccccccccc}
\toprule
&&\texttt{0-shot} & &&& &\texttt{few-shot}$^*$ & \vspace{1mm} \\

 & \texttt{Poly} & \texttt{Poly}-$\mu$ & \shared{}  &&& \texttt{Poly} & \texttt{Poly}-$\mu$ & \shared{} \\
\midrule   
Avg & \textbf{55.4} & 55.3 &54.3  &&& 64.5 & \textbf{65.2} & 65.2 &\\
\bottomrule
\end{tabular}
\caption{Results in the $\texttt{zero-shot}$ and $\texttt{few-shot}$ setting for the T0 dataset. The asterisk is meant to denote that we fine-tune all models for 1000 steps on the training set of the test tasks, given the lack of a validation set. This setting is the default in the \texttt{T-Few} paper and thus we suspect it benefits \texttt{T-Few}.}
% \end{tabular}
\end{table*}

==> old_tables/t0_table.tex <==
\begin{table*}[t]
% \vspace{-10pt}
\centering
\small
\begin{tabular}{l|r|rrr}
\toprule
T0 Task & \texttt{Shared} &\polym{} &\poly{} &\polys{} \\
\midrule
\textsc{anli-r1} &49.1$_{0.7}$  &49.8$_{0.8}$  &49.9$_{0.9}$  &49.9$_{2.2}$  \\
\textsc{anli-r2} &43.5$_{1.6}$  &42.9$_{2.1}$  &43.4$_{2.2}$  &42.9$_{1.9}$  \\
\textsc{anli-r3} &40.5$_{3.2}$  &40.8$_{3.1}$  &41.2$_{4.2}$  &40.8$_{5.0}$  \\
\textsc{cb} &91.1$_{3.6}$  &91.1$_{1.8}$  &91.1$_{1.8}$  &92.9$_{1.8}$  \\
\textsc{copa} &90.0$_{6.0}$  &90.0$_{5.0}$  &90.0$_{6.0}$  &90.0$_{4.0}$  \\
\textsc{h-swag} &51.8$_{4.9}$  &52.1$_{5.1}$  &54.7$_{0.0}$  &52.6$_{3.3}$  \\
\textsc{rte} &82.3$_{0.4}$  &81.2$_{1.8}$  &80.9$_{2.9}$  &83.0$_{2.9}$  \\
\textsc{storycloze} &95.6$_{2.2}$  &95.4$_{1.5}$  &95.2$_{1.7}$  &96.0$_{2.1}$  \\
\textsc{wic} &57.2$_{1.3}$  &57.4$_{3.9}$  &57.8$_{2.7}$  &58.3$_{3.4}$  \\
\textsc{winogrande} &62.3$_{1.9}$  &61.8$_{0.6}$  &62.1$_{0.8}$  &62.4$_{1.7}$  \\
\textsc{wsc} &72.1$_{1.0}$  &73.1$_{3.8}$  &72.1$_{5.8}$  &73.1$_{3.8}$  \\
\midrule
Avg$^*$ & 66.9$_{0.7}$  & 67.2$_{1.1}$  & 67.1$_{1.4}$ & \underline{67.5}$^{\uparrow0.6}_{0.5}$   \\
\bottomrule


\end{tabular}
\caption{Results on the 11 test tasks of the T0 data. We report the median and interquartile range computed over 5 seeds. The asterix is meant to denote the lack of proper evaluation framework due to the lack of validation set. To ensure fairness for all methods, we report the best validation accuracy per task, evaluated every 4 fine-tuning epochs.}
\label{tab:t0}
\end{table*}

==> old_tables/xfit_bigtable.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lc|r|rrrr|r}
\toprule
Crossfit Task & Metric &\texttt{Shared} &\private{} &\random{} &\polym{} &\poly{} &\polys{} \\
\midrule
\textsc{ag-news} & \textsc{C--F1} & 81.5$_{1.3}$  &71.3$_{7.1}$  &83.3$_{2.3}$  &85.1$_{1.3}$  &85.0$_{2.1}$  &84.4$_{1.5}$  \\
\textsc{ai2-arc} & \textsc{Acc} & 27.2$_{2.1}$  &22.9$_{2.4}$  &24.7$_{1.3}$  &24.2$_{3.3}$  &24.0$_{2.2}$  &25.8$_{3.4}$  \\
\textsc{amzn-polarity} & \textsc{C--F1} & 87.6$_{14.4}$  &78.5$_{22.5}$  &93.0$_{0.8}$  &92.4$_{2.0}$  &92.7$_{1.9}$  &93.6$_{1.0}$  \\
\textsc{bsn-npi-present} & \textsc{Acc} & 99.2$_{0.4}$  &100.0$_{0.0}$  &99.2$_{0.4}$  &99.6$_{0.2}$  &99.1$_{0.5}$  &98.7$_{1.3}$  \\
\textsc{bsn-npi-scope} & \textsc{Acc} & 99.9$_{0.2}$  &99.6$_{0.9}$  &100.0$_{0.0}$  &99.4$_{0.9}$  &99.6$_{0.7}$  &99.7$_{0.3}$  \\
\textsc{break-qdmr} & \textsc{EM} & 3.9$_{0.8}$  &3.0$_{1.5}$  &2.6$_{1.5}$  &3.5$_{1.0}$  &4.1$_{0.5}$  &3.3$_{2.0}$  \\
\textsc{circa} & \textsc{C--F1} & 46.4$_{4.7}$  &31.2$_{7.9}$  &47.3$_{5.2}$  &45.4$_{4.7}$  &43.5$_{6.4}$  &47.6$_{5.6}$  \\
\textsc{crawl-domain} & \textsc{EM} & 40.0$_{3.0}$  &42.9$_{3.7}$  &43.9$_{2.0}$  &47.3$_{1.3}$  &45.0$_{4.2}$  &46.2$_{2.1}$  \\
\textsc{ethos-disab.} & \textsc{C--F1} & 69.9$_{9.9}$  &54.0$_{6.5}$  &60.6$_{8.6}$  &73.4$_{9.8}$  &74.0$_{10.3}$  &73.5$_{8.1}$  \\
\textsc{ethos-sexual} & \textsc{C--F1} & 65.0$_{9.7}$  &52.3$_{15.5}$  &58.9$_{16.1}$  &81.4$_{9.6}$  &78.9$_{4.5}$  &84.0$_{6.3}$  \\
\textsc{freebase-qa} & \textsc{EM} & 2.7$_{1.0}$  &0.1$_{0.2}$  &5.4$_{0.6}$  &3.9$_{1.7}$  &3.8$_{1.5}$  &3.9$_{1.7}$  \\
\textsc{glue-cola} & \textsc{M-Cor} & 6.8$_{4.4}$  &9.5$_{5.7}$  &7.9$_{6.8}$  &8.2$_{5.6}$  &7.5$_{11.6}$  &9.9$_{8.8}$  \\
\textsc{glue-qnli} & \textsc{Acc} & 74.0$_{2.4}$  &55.3$_{2.8}$  &75.2$_{3.4}$  &72.3$_{5.0}$  &73.1$_{4.4}$  &75.5$_{4.4}$  \\
\textsc{hatexplain} & \textsc{C--F1} & 43.6$_{3.3}$  &33.3$_{3.9}$  &43.8$_{2.4}$  &42.2$_{4.1}$  &44.3$_{2.5}$  &41.3$_{6.4}$  \\
\textsc{quoref} & \textsc{QA--F1} & 43.8$_{2.8}$  &33.5$_{3.1}$  &44.6$_{4.3}$  &46.3$_{2.2}$  &45.0$_{3.9}$  &44.9$_{2.6}$  \\
\textsc{race-high} & \textsc{Acc} & 34.9$_{1.0}$  &26.0$_{1.7}$  &34.0$_{2.9}$  &33.0$_{0.7}$  &32.4$_{1.5}$  &32.5$_{3.1}$  \\
\textsc{superglue-rte} & \textsc{Acc} & 60.1$_{3.2}$  &47.8$_{2.2}$  &57.7$_{3.7}$  &52.0$_{3.3}$  &52.3$_{3.8}$  &60.2$_{3.8}$  \\
\textsc{tw.-eval-irony} & \textsc{C--F1} & 56.7$_{3.0}$  &46.0$_{7.5}$  &57.2$_{2.2}$  &55.6$_{1.4}$  &54.8$_{1.7}$  &56.4$_{3.2}$  \\
\textsc{wiki-split} & \textsc{R-L} & 80.3$_{0.5}$  &80.7$_{0.3}$  &80.3$_{0.5}$  &79.8$_{1.0}$  &80.2$_{0.3}$  &80.3$_{0.6}$  \\
\textsc{yelp-polarity} & \textsc{C--F1} & 94.8$_{0.8}$  &55.2$_{11.9}$  &94.4$_{0.4}$  &95.1$_{0.5}$  &94.9$_{0.4}$  &95.5$_{0.3}$  \\
\midrule
All & Avg & 55.9$_{0.7}$  &47.2$_{1.6}$  &55.7$_{1.4}$  &57.0$_{0.5}$  &56.7$_{0.4}$  &\underline{57.8}$^{\uparrow1.9}_{0.5}$ \\
\bottomrule

\end{tabular}
\caption{Results on the \texttt{CrossFit} test tasks. \texttt{Shared} does multi-task training of one shared LoRA and fine-tunes it for each test task; \texttt{Poly} learns both the routing matrix $Z$ and fine-tunes skills $\Phi$; \polym{} fine-tunes the average of skills learnt with \texttt{Poly}; \texttt{Random}-$\mu$ fine-tunes the average of skills learnt during multi-task training with a random fixed $Z$; \texttt{Private}-$\mu$ first train on skill per training task, and then fine-tunes the average of private skills. In \texttt{CrossFit}, most of the \poly{} gain comes from the effective initialization while learning the routing vector $z_{\tau}$ for the downstream tasks seems unnecessary. \polys{} improve over all baselines. The superscript in the last line reports the improvement of \polys{} w.r.t. \shared{}.}
\label{tab:xfit}
\end{table*}

==> tables/ablate_and_polymu.tex <==
\begin{table}[t]
\fontsize{11}{13}\selectfont    
\centering

\begin{minipage}{0.5\textwidth}
% \vspace{3pt}
\begin{tabular}{lcccc}
\toprule
\textbf{T0 Dataset} & \textbf{Test Acc.} \\
\midrule
% \poly{} (\texttt{LoRA}) & 68.0$_{1.0}$ \\
\shared{} (\texttt{LoRA}) & 66.0$_{1.5}$ \\
% \texttt{Random}-$\mu$ (\texttt{LoRA}) & 66.0$_{1.6}$ \\
% \texttt{Private} (refined) & 56.3$_{0.8}$ \\
% \texttt{Private} (coarse)  & 61.0$_{0.1}$ \\
\midrule
{\emph{Uniform Aggregation}} &  \\
\texttt{AdapterSoup}-$\mu$ (refined) & 56.3$_{0.8}$ \\
\texttt{AdapterSoup}-$\mu$ (coarse)  & 61.0$_{0.1}$ \\
\midrule
{\emph{Similarity Aggregation}} &  \\
\texttt{AdapterSoup} (coarse, k=1)  & 60.7$_{1.1}$ \\
\texttt{AdapterSoup} (coarse, k=5)  & 62.1$_{1.0}$ \\

\bottomrule
\end{tabular}
% \captionsetup{width=1.1\linewidth}
\caption{Evaluation of Transfer and Interference during Multi-Task Pretraining. We compare methods sharing \textit{all} parameters across tasks ($\texttt{LoRA}$), with those sharing none (\AS{}).}
\label{tab:ablate_one}
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.45\textwidth}

\hspace{2mm}
\begin{tabular}{lcccc}
\toprule
\textbf{T0 Dataset} & \textbf{Test Acc.} \\
\midrule
\poly{} & 68.0$_{0.8}$ \\
\polys{} & 69.1$_{1.1}$ \\
\polym{} & 67.8$_{0.6}$ \\
\polysm{} & 69.1$_{0.9}$ \\
\midrule
\textbf{SuperNI} & \textbf{Test Rouge-L} \\
\midrule
\poly{} & 67.7$_{0.2}$ \\
\polys{} & 68.5$_{0.6}$ \\
\polym{}  & 68.2$_{0.6}$ \\
\polysm{} & 68.5$_{0.2}$ \\
\bottomrule
\end{tabular}
\vspace{1mm}

% \captionsetup{width=0.8\linewidth}
\caption{Evaluating the impact of modular adaptation at test time.}
\label{tab:poly_mu}
\end{minipage}
\end{table}


==> tables/ablation_table.tex <==
\begin{wraptable}[16]{t}{0.50\textwidth}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Test Acc.} \\
\midrule

\shared{} & 66.04$_{1.6}$ \\
\cdashlinelr{1-2}
\rowcolor{lightgray}{\emph{Uniform Aggregation}} &  \\
\texttt{AdapterSoup} (refined) & 56.30$_{0.8}$ \\
\texttt{AdapterSoup} (coarse)  & 61.02$_{0.1}$ \\
\cdashlinelr{1-2}
\rowcolor{lightgray}{\emph{Similarity Aggregation}} &  \\
\texttt{AdapterSoup} (coarse, k=1)  & 60.71$_{1.1}$ \\
\texttt{AdapterSoup} (coarse, k=5)  & 62.07$_{1.0}$ \\

\bottomrule
\end{tabular}
\label{tab:private}
\caption{Comparison of methods that sharing all parameters with methods training separate parameters per task.}
\end{wraptable}

==> tables/ale_ni_table.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Model} &  Multi-Task Params & Adaptation Params & Avg. Test Accuracy \\
\midrule
\texttt{ia3} & 540K & 540K & - \\
\AS{} & 84M & 2.2M & 62.1$_{1.0}$ \\
\texttt{LoRA}  & 2.2M & 2.2M & 66.0$_{1.6}$ \\
\texttt{LoRA-big} & 35M  & 35M  & 65.4$_{0.9}$  \\ 
\poly{}-$z$ & 17M & 3.5K & 66.4$_{0.3}$ \\
\poly{} & 17M & 2.2M & 68.0$_{1.0}$ \\
\midrule
% \polys{} \emph{(8 h)} & 17M & 2.2M & 68.1$_{0.7}$ \\
\polys{}$z$ & 17M & 220K & 68.3$_{0.8}$ \\
\polys{} & 17M & 2.2M & \underline{69.1}$_{1.0}$ \\
\midrule
\midrule
\label{tab:ni_results}
\end{tabular}
\caption{Results on T0 dataset \cite{sanh2022multitask}, we report the mean of the best validation accuracy for each test task, when evaluated every 50 train epochs. \tfew{} is our reproduction of the results in~\cite{tfew}. \texttt{LoRA-big} means a \texttt{LoRA} adapter with a larger rank.}
\hspace{0.01\textwidth}
\end{table}


==> tables/ale_table.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Model} &  Multi-Task Params & Adaptation Params & Avg. Test \\
\midrule
\multicolumn{4}{l}{\textbf{T0 Dataset}}
\\
\midrule
\multicolumn{4}{l}{\emph{Backbone T5-XL-LM}} \\
\texttt{ia3} \cite{tfew} & 540K & 540K & 62.4$_{0.4}$ \\
\AS{} & 84M & 2.2M & 62.1$_{1.0}$ \\
\texttt{LoRA}  & 2.2M & 2.2M & 66.0$_{1.6}$ \\
\texttt{LoRA-big} & 35M  & 35M  & 65.4$_{0.9}$  \\ 
\poly{}-$z$ & 17M & 3.5K & 66.4$_{0.3}
$ \\
\poly{} & 17M & 2.2M & 68.0$_{1.0}$ \\
% \polys{} \emph{(8 h)} & 17M & 2.2M & 68.1$_{0.7}$ \\
\rowcolor{lightgray}\polys{}-$z$ & 17M & 220K & 68.3$_{0.8}$ \\
\rowcolor{lightgray}\polys{} & 17M & 2.2M & \underline{69.1}$_{1.0}$ \\
\midrule
\multicolumn{4}{l}{\emph{Backbone T0-3B}} \\
\tfew~\cite{tfew} & 540K & 540K & 66.2$_{0.5}$ \\
% \emph{l}-\texttt{LoRA}~\emph{(rank 1)} & 934K  & 934K & 66.2$_{0.9}$  \\
% \emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 15M  & 15M  & 67.6$_{1.1}$  \\
% \AS{} (\emph{l}-\texttt{LoRA}) & X & X & x & x \\
% \emph{l}-\poly{} & 7.5M & 934K & 68.0$_{0.5}$ \\
\AS{} & 84M & 2.2M & 66.1$_{0.6}$ \\
\texttt{LoRA}  & 2.2M & 2.2M & 67.4$_{0.8}$ \\
\texttt{LoRA-big} & 35M  & 35M  &  -  \\ 
\poly{}-$z$ & 17M & 3.5K & 65.3$_{1.0}$  \\
\poly{} & 17M & 2.2M & 69.0$_{0.8}$ \\
% \polys{} \emph{(8 h)} & 17M & 2.2M & 68.1$_{0.7}$ \\
\rowcolor{lightgray}\polys{}$z$ & 17M & 220K & 68.4$_{1.2}$  \\
\rowcolor{lightgray}\polys{} & 17M & 2.2M & 69.3$_{1.2}$ \\
% \emph{l}-\polys{} & 7.5M & 934K & \underline{68.5}$_{0.7}$ \\
% \emph{l}-\polys{} \emph{(64 h)} & 7.5M & 934K & 67.6$_{0.9}$ \\
\midrule
\midrule
\multicolumn{4}{l}{\textbf{SuperNI Dataset}} \\
\midrule
\multicolumn{4}{l}{\emph{Backbone T5-XL-LM}} \\
\texttt{LoRA}  & 2.2M & 2.2M &  \\
\texttt{LoRA-big}
 & 35M  & 35M & \\ 
\poly{}-$z$ & 17M & 3.5K & \\
\poly{} & 17M & 2.2M & \\
\midrule
\polys{}$z$ & 17M & 220K & \\
\polys{} & 17M & 2.2M &  \\
\bottomrule
\label{tab:t0_results}
%\label{tab:ni_results}
\end{tabular}
\caption{(top) Results on T0 dataset \cite{sanh2022multitask}, we report the mean of the best validation accuracy for each test task, when evaluated every 50 train epochs. \tfew{} is our reproduction of the results in~\cite{tfew}. \texttt{LoRA-big} means a \texttt{LoRA} adapter with a larger rank. (bottom) Results on SuperNatural Instructions dataset. \textcolor{red}{write what is Subscripts}}

\hspace{0.01\textwidth}

\end{table}


==> tables/larger_t0_table.tex <==

\begin{table}[t]
\hspace{-10pt}

\begin{tabular}{ll@{\hskip.2in}cc@{\hskip.2in}cc}
\toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{\#Params}} & \textbf{Test Acc.} \\
\multicolumn{2}{c}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Standard Tuning } {\hskip.5in}} & \multicolumn{2}{c}{\textbf{Z-tuning only}} \\
\multicolumn{2}{c}{Approach \ \ Shared Params} & Test Params & Accuracy &  Test Params & Accuracy  \\
\midrule
\rowcolor{lightgray}\multicolumn{6}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\texttt{LoRA}  & 2.2M & 2.2M & 66.0$_{1.6}$ & - & - \\
% \texttt{LoRA}~\emph{(rank 16)} & 35M  & 35M  & 65.4$_{0.9}$ & - & - \\ 
\texttt{LoRA-big} & 71M  & 71M  & 67.0$_{1.0}$ & - & - \\
\AS{} (\texttt{LoRA}) & 84M & 2.2M & 62.1$_{1.0}$ & - & - \\
\poly{} & 17M & 2.2M & 68.0$_{1.0}$ & 3.5K & 66.4$_{0.3}$ \\
% \polys{} \emph{(8 h)} & 17M & 2.2M & 68.1$_{0.7}$ & 13.3K & 67.9$_{0.1}$ \\
\polys{} & 17M & 2.2M & \underline{69.1}$_{1.0}$ & 220K & 68.3$_{0.8}$ \\
\midrule
\texttt{Full-FT}+\texttt{LoRA} & 3.9B & 2.2M & 68.9$_{1.4}$ & - & - \\
\midrule
\rowcolor{lightgray}\multicolumn{6}{l}{\textbf{\emph{Backbone T0-3B}}} \\
% \tfew{} \cite{tfew} & 545K & 545K & 66.9$_{0.7}$ & - & - \\
\tfew~\cite{tfew} & 540K & 540K & 66.2$_{0.5}$ & - & - \\
\emph{l}-\texttt{LoRA}~\emph{(rank 1)} & 934K  & 934K & 66.2$_{0.9}$  & - & - \\
\emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 15M  & 15M  & 67.6$_{1.1}$ & - & - \\
\AS{} (\emph{l}-\texttt{LoRA}) & 35M & 934K &64.9$_{1.0}$ & - & - 
\vspace{3.5pt} \\
\emph{l}-\poly{} & 7.5M & 934K & 68.0$_{0.5}$ & - & -  \\
\emph{l}-\polys{} \emph{(8 h)} & 7.5M & 934K & \underline{68.5}$_{0.7}$ & - & -  \\
\emph{l}-\polys{} \emph{(64 h)} & 7.5M & 934K & 67.6$_{0.9}$ & - & -  \\

% The following are the full LoRA / Poly on T0-3B. Uncomment for now
% \cdashlinelr{1-6}
% \texttt{LoRA}~\emph{(rank 1)}  & 2.2M & 2.2M & X & - & - \\
% \texttt{LoRA}~\emph{(rank 16)} 
% & 35M  & 35M  & X & - & - 
% \vspace{3.5pt} \\
% \poly{} & 17M & 2.2M & X & - & -  \\
% \polys{} \emph{(64 h)} & 17M & 2.2M & 68.39 & - & -  \\

\bottomrule
\label{tab:t0_results}
\end{tabular}
\caption{Results on T0 dataset \cite{sanh2022multitask}, we report the mean of the best validation accuracy for each test task, when evaluated every 50 train epochs. \tfew{} is our reproduction of the results in~\cite{tfew}.}

\hspace{0.01\textwidth}

\end{table}


==> tables/ni_table.tex <==

\begin{table}[t]
\hspace{-10pt}
\centering
\begin{tabular}{ll@{\hskip.2in}cc@{\hskip.2in}cc}
\toprule
\multicolumn{2}{c}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Standard Tuning } {\hskip.5in}} & \multicolumn{2}{c}{\textbf{Z-tuning only}} \\
\multicolumn{2}{c}{Approach \ \ Train Params} & Test Params & Rouge-L &  Test Params & Rouge-L  \\
\midrule
\rowcolor{lightgray}\multicolumn{6}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
% \midrule
\texttt{LoRA}~\emph{(rank 16)} & 18M  & XM  & 68.5$_{0.9}$ & - & - \\ 
\cdashlinelr{1-6}
\poly{} & 7.5M & 18M & 68.6$_{0.8}$ & XK & 65.4$_{0.3}$ \\
\polys{} \emph{(8 h)} & 7.5M & XM & \underline{69.4}$_{0.3}$ & XK & 68.4$_{0.3}$ \\
% \polys{} \emph{(64 h)} & 7.5M & XM & 68.9$_{0.6}$ & XK & 69.0$_{0.4}$ \\

\bottomrule
\end{tabular}

\caption{Results on Natural Instructions dataset \cite{ni}}
\label{tab:ni}
\hspace{0.01\textwidth}

\end{table}


==> tables/ni_table_wrap.tex <==
\begin{wrapfigure}{l}{0.56\textwidth}
\begin{tabular}{lcc}

\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\multicolumn{3}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\midrule

\emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 18M / 18M & 68.53$_{0.9}$ \\

\cdashlinelr{1-3}
\poly{} & 7.5M / 18M & 68.6$_{0.8}$ \\
\polys{} \emph{(8 h)} & 7.5M / 18M & 69.4$_{0.3}$ \\
\polys{} \emph{(64 h)} & 7.5M / 18M & 68.9$_{0.6}$  \\
\midrule
\rowcolor{lightgray}\emph{$Z$-tuning} & & \\
\poly{} & 7.5M / \ 2.1K  & 65.37$_{0.3}$ \\
\polys{} \emph{(8 h)} & 7.5M / 13.3K  & 68.40$_{0.3}$ \\
\polys{} \emph{(64 h)} & 7.5M / 147K & 69.00$_{0.4}$ \\
\bottomrule

\end{tabular}
\caption{SuperNatural Instruction \cite{ni} results.}

% \caption{Results on T0 dataset, starting from the T0-3B model. To be comparable with~\citep{tfew}, we train a ``light'' version of our \texttt{LoRA} based models, prefixed with \emph{l-}, where we only patch \texttt{k,v,wi1} layers as \tfew{}.}
\end{wrapfigure}



==> tables/polymu_table.tex <==
\begin{table}[hbp]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Test Acc.} \\
\midrule
\rowcolor{lightgray}{\emph{Natural Instructions}} &  \\
\poly{} & 68.6$_{0.8}$ \\
\poly{}$-\mu$  & 69.2$_{0.6}$ \\
\polys{} \emph{(64 h)} & 68.9$_{0.6}$ \\
\polys{} \emph{(64 h)} $-\mu$  & 68.5$_{0.8}$ \\
\cdashlinelr{1-2}
\rowcolor{lightgray}{\emph{T0 Dataset}} &  \\
\poly{} & 68.0$_{0.8}$ \\
\poly{}$-\mu$  & 67.8$_{0.6}$ \\
\polys{} \emph{(64 h)} & 69.1$_{1.1}$ \\
\polys{} \emph{(64 h)} $-\mu$  & 69.1$_{0.9}$ \\
\bottomrule
\end{tabular}

\caption{Ablation}
\end{table}

==> tables/small_ni_dataset.tex <==
\textbf{SuperNI Dataset} & \textbf{Rouge-L} \\
\midrule
\texttt{Full-FT} + \texttt{(IA)}$^3$ & 68.0$_{0.8}$ \\
\texttt{Full-FT} + \texttt{LoRA} & 67.9$_{0.7}$ \\
\texttt{LoRA}  &  67.6$_{0.8}$ \\
\texttt{LoRA-big} & 67.2$_{0.7}$ \\ 
\poly{}-$z$ &  64.6$_{0.3}$\\
\poly{} &  67.8$_{0.8}$\\
\rowcolor{lightgray}\polys{}-$z$   & 68.0$_{0.2}$\\
\rowcolor{lightgray}\polys{} & \underline{68.5}$_{0.3}$ \\

==> tables/small_t03b_table.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Model} &  Avg. Test \\
\midrule
\multicolumn{2}{l}{\emph{Backbone T0-3B}} \\
\tfew~\cite{tfew} & 66.2$_{0.5}$ \\
\AS{} &  66.1$_{0.6}$ \\
\texttt{LoRA}  &  67.4$_{0.8}$ \\
\texttt{LoRA-big} &  &  -  \\ 
\poly{}-$z$  & 65.3$_{1.0}$  \\
\poly{} &  69.0$_{0.8}$ \\
\rowcolor{lightgray}\polys{}$z$ \emph{(8 h)} & 68.4$_{1.2}$  \\
\rowcolor{lightgray}\polys{} \emph{(64 h)} &  69.3$_{1.2}$ \\
\bottomrule
\label{tab:small_t0_table}
\end{tabular}
\caption{Results on T0 dataset \cite{sanh2022multitask}, we report the mean of the best validation accuracy for each test task, when evaluated every 50 train epochs.}
\end{table}


==> tables/t0_ni_table.tex <==
\begin{table}[t]
\fontsize{9.3}{11}\selectfont    
\centering
\begin{minipage}{0.48\textwidth}
\vspace{-4pt}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\multicolumn{3}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\midrule
% \tfew{} (Raffel, 2022) & 2.9B & 545K & 66.90 & 0.70 \\
% \tfew{} (\emph{Ours}) & 2.9B & 545K & 69.20 & 0.68 \\
\texttt{LoRA}~\emph{(rank 1)} & 2.2M / 2.2M & 66.04$_{1.6}$ \\
% \texttt{LoRA}~\emph{(rank 16)} & 35M / 35M & 65.43$_{0.9}$ \\
% \texttt{LoRA}\texttt{[r=16]} & 35.4M & 35.4M & 65.43 & 0.99 \\
% \texttt{LoRA}\texttt{[r=32]} & 70.8M & 70.8M & 66.98 & 0.99 \\
\cdashlinelr{1-3}
\poly{} & 17M / 2.2M & 67.96$_{1.0}$ \\
% \poly{}\texttt{[s=8]} & 17.7M & 2.2M & 67.96 & 1.03 \\
% \poly{}\texttt{[s=32]} & 70.8M & 2.2M & 67.76 & 1.04 \\
% \poly{}\texttt{[s=8,h=8]} & 17.7M & 2.2M & 68.13 & 0.75 \\
% \poly{}\texttt{[s=8,h=32]} & 17.7M & 2.2M & 68.41 & 1.40 \\
% \poly{}\texttt{[s=8,h=64]} & 17.7M & 2.2M & 69.14 & 1.05 \\
\polys{} \emph{(8 h)} & 17M / 2.2M & 68.13$_{0.7}$ \\
% \polys{} \emph{(32 h)} & 17M / 2.2M & 68.41$_{1.4}$ \\
\polys{} \emph{(64 h)} & 17M / 2.2M & \underline{69.14}$_{1.0}$ \\
\midrule
\rowcolor{lightgray}\emph{$Z$-tuning only} & & \\
\poly{} & 17M / 3.5K  & 66.38$_{0.3}$ \\
\polys{} \emph{(8 h)} &  ? M / 13.3K  & 67.89$_{0.1}$ \\
\polys{} \emph{(64 h)} & 17M / 220K  & 68.25$_{0.8}$ \\
% \cdashlinelr{1-3}
% $Z$-tune \emph{(64h bw)} & 17M / 24.6K & 68.17$_{0.8}$ \\
\bottomrule
\end{tabular}
%\label{tab:t0_table}
% \vspace{15pt}
\caption{Results on T0 dataset \cite{sanh2022multitask}}
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.48\textwidth}

\begin{tabular}{lcc}

\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\multicolumn{3}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\midrule

\emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 18M / 18M & 68.53$_{0.9}$ \\

\cdashlinelr{1-3}
\poly{} & 7.5M / 18M & 68.6$_{0.8}$ \\
\polys{} \emph{(8 h)} & 7.5M / 18M & 69.4$_{0.3}$ \\
\polys{} \emph{(64 h)} & 7.5M / 18M & 68.9$_{0.6}$  \\
\midrule
\rowcolor{lightgray}\emph{$Z$-tuning} & & \\
\poly{} & 7.5M / \ 2.1K  & 65.37$_{0.3}$ \\
\polys{} \emph{(8 h)} & 7.5M / 13.3K  & 68.40$_{0.3}$ \\
\polys{} \emph{(64 h)} & 7.5M / 147K & 69.00$_{0.4}$ \\
\bottomrule

\end{tabular}



\caption{Results on SuperNatural Instruction \cite{ni}}


\end{minipage}

\vspace{5pt}

% \caption{Results on T0 dataset, starting from the T0-3B model. To be comparable with~\citep{tfew}, we train a ``light'' version of our \texttt{LoRA} based models, prefixed with \emph{l-}, where we only patch \texttt{k,v,wi1} layers as \tfew{}.}
\end{table}

==> tables/t0_table.tex <==
\begin{table}[t]
\fontsize{9.3}{11}\selectfont    
\centering
\begin{minipage}{0.48\textwidth}
\vspace{-4pt}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\multicolumn{3}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\midrule
% \tfew{} (Raffel, 2022) & 2.9B & 545K & 66.90 & 0.70 \\
% \tfew{} (\emph{Ours}) & 2.9B & 545K & 69.20 & 0.68 \\
\texttt{LoRA}~\emph{(rank 1)} & 2.2M / 2.2M & 66.04$_{1.6}$ \\
\texttt{LoRA}~\emph{(rank 16)} & 35M / 35M & 65.43$_{0.9}$ \\
% \texttt{LoRA}\texttt{[r=16]} & 35.4M & 35.4M & 65.43 & 0.99 \\
% \texttt{LoRA}\texttt{[r=32]} & 70.8M & 70.8M & 66.98 & 0.99 \\
\cdashlinelr{1-3}
\poly{} & 17M / 2.2M & 67.96$_{1.0}$ \\
% \poly{}\texttt{[s=8]} & 17.7M & 2.2M & 67.96 & 1.03 \\
% \poly{}\texttt{[s=32]} & 70.8M & 2.2M & 67.76 & 1.04 \\
% \poly{}\texttt{[s=8,h=8]} & 17.7M & 2.2M & 68.13 & 0.75 \\
% \poly{}\texttt{[s=8,h=32]} & 17.7M & 2.2M & 68.41 & 1.40 \\
% \poly{}\texttt{[s=8,h=64]} & 17.7M & 2.2M & 69.14 & 1.05 \\
\polys{} \emph{(8 h)} & 17M / 2.2M & 68.13$_{0.7}$ \\
\polys{} \emph{(32 h)} & 17M / 2.2M & 68.41$_{1.4}$ \\
\polys{} \emph{(64 h)} & 17M / 2.2M & \underline{69.14}$_{1.0}$ \\
\midrule
\rowcolor{lightgray}\emph{$Z$-tuning only} & & \\
\poly{} & 17M / 3.5K  & 66.38$_{0.3}$ \\
\polys{} \emph{(64 h)} & 17M / 220K  & 68.25$_{0.8}$ \\
% \cdashlinelr{1-3}
% $Z$-tune \emph{(64h bw)} & 17M / 24.6K & 68.17$_{0.8}$ \\
\bottomrule
\end{tabular}
%\label{tab:t0_table}
% \vspace{15pt}
\caption{Results on T0 dataset, starting from T5-XL-LM 3B model.}
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.48\textwidth}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\textbf{\emph{Backbone T0-3B}} & &\\
% \tfew{} (\emph{Ours}) & 2.9B & 545K & 69.20 & 0.68 \\
\midrule
\tfew{}
%~\citep{tfew} 
& 545K / 545K & 66.90$_{0.7}$ \\
\emph{l}-\texttt{LoRA}~\emph{(rank 1)} & 934K / 934K & 66.21$_{0.9}$ \\
\emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 35M / 35M & 67.57$_{1.1}$\\
% \texttt{LoRA}\texttt{[r=16]} & 35.4M & 35.4M & 65.43 & 0.99 \\
% \texttt{LoRA}\texttt{[r=32]} & 70.8M & 70.8M & 66.98 & 0.99 \\
\cdashlinelr{1-4}
\emph{l}-\poly{} & 7.5M / 934K & 68.02$_{0.5}$ \\
\emph{l}-\polys{} \emph{(8 h)} & 7.5M / 934K & \underline{68.47}$_{0.7}$ \\
\emph{l}-\polys{} \emph{(64 h)} & 7.5M / 934K & 67.57$_{0.9}$ \\
\cdashlinelr{1-4}
\poly{} & 17M / 2.2M & 69.53$_{0.6}$ \\
\polys{} \emph{(8 h)} & 17M / 2.2M & x \\
\polys{} \emph{(64 h)} & 17M / 2.2M & \underline{70.35}$_{1.0}$ \\
\bottomrule
\end{tabular}

\caption{Results on T0 dataset, starting from T0-3B model.}
\end{minipage}
\vspace{5pt}

% \caption{Results on T0 dataset, starting from the T0-3B model. To be comparable with~\citep{tfew}, we train a ``light'' version of our \texttt{LoRA} based models, prefixed with \emph{l-}, where we only patch \texttt{k,v,wi1} layers as \tfew{}.}
\end{table}

==> tables/xfit_ni_table.tex <==
\begin{table}[t]
\fontsize{9.3}{11}\selectfont    
\centering
\begin{minipage}{0.48\textwidth}
\hspace{-10pt}
\begin{tabular}{lcc}

\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\multicolumn{3}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\midrule

\emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 142M / 18M & 66.45$_{1.3}$ \\

\cdashlinelr{1-3}
\emph{l}-\poly{} & 142M / 18M & 66.27$_{1.4}$ \\

\emph{l}-\poly{} \emph{(8 h)} & 142M / 18M & 66.24$_{1.1}$ \\
\emph{l}-\poly{} \emph{(64 h)} & 142M / 18M & 66.32$_{0.1}$ \\

\midrule
\rowcolor{lightgray}\emph{$Z$-tuning} & & \\
\poly{} & 142M / \ 2.1K  & 55.90$_{0.9}$ \\
\polys{} \emph{(8 h)} & 142M / 13.3K  & 63.74$_{0.9}$ \\
\polys{} \emph{(64 h)}& 142M / 147K & 66.03$_{0.9}$ \\

\bottomrule

\end{tabular}
\caption{Crossfit \cite{xfit} Benchmark Results}
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.48\textwidth}

\begin{tabular}{lcc}

\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{Test Acc.} \\
 &  MT / Test &  \\
\midrule
\rowcolor{lightgray}\multicolumn{3}{l}{\textbf{\emph{Backbone T5-XL-LM}}} \\
\midrule

\emph{l}-\texttt{LoRA}~\emph{(rank 16)} & 18M / 18M & 68.53$_{0.9}$ \\

\cdashlinelr{1-3}
\poly{} & 7.5M / 18M & 68.6$_{0.8}$ \\
\polys{} \emph{(8 h)} & 7.5M / 18M & 69.4$_{0.3}$ \\
\polys{} \emph{(64 h)} & 7.5M / 18M & 68.9$_{0.6}$  \\
\midrule
\rowcolor{lightgray}\emph{$Z$-tuning} & & \\
\poly{} & 7.5M / \ 2.1K  & 65.37$_{0.3}$ \\
\polys{} \emph{(8 h)} & 7.5M / 13.3K  & 68.40$_{0.3}$ \\
\polys{} \emph{(64 h)} & 7.5M / 147K & 69.00$_{0.4}$ \\
\bottomrule

\end{tabular}


\label{tab:t0_table}
\caption{SuperNatural Instruction \cite{ni} results.}
\end{minipage}
\vspace{5pt}

% \caption{Results on T0 dataset, starting from the T0-3B model. To be comparable with~\citep{tfew}, we train a ``light'' version of our \texttt{LoRA} based models, prefixed with \emph{l-}, where we only patch \texttt{k,v,wi1} layers as \tfew{}.}
\end{table}
